On the Parallel Complexity of Multilevel Monte Carlo in Stochastic Gradient Descent

In the stochastic gradient descent (SGD) for sequential simulations such as the neural stochastic differential equations, the Multilevel Monte Carlo (MLMC) method is known to offer better theoretical computational complexity compared to the naive Monte Carlo approach. However, in practice, MLMC scales poorly on massively parallel computing platforms such as modern GPUs, because of its large parallel complexity which is equivalent to that of the naive Monte Carlo method. To cope with this issue, we propose the delayed MLMC gradient estimator that drastically reduces the parallel complexity of MLMC by recycling previously computed gradient components from earlier steps of SGD. The proposed estimator provably reduces the average parallel complexity per iteration at the cost of a slightly worse per-iteration convergence rate. In our numerical experiments, we use an example of deep hedging to demonstrate the superior parallel complexity of our method compared to the standard MLMC in SGD.

==> note.tex <==

\begin{remark}[Personal Notes]
When $\Delta_\ell \hat F(x, \xi)$ is not smooth, we should still be able to prove the smoothness of its expectation $F(x)$ under some regularity conditions.

In the case of neural SDEs, Assumption \ref{assum:smoothness} follows if the analytical solution of the SDE (i.e. $\hat F_\infty (x, \xi)= \Lcal(X_T)$) has the strong convergence of order $1$ for the gradient of Milstein scheme. When the stochastic adjoint method \citep{scalable-sde} is used to calculate the gradient we get the desired strong order $1$. From our experience, backpropagation through a solver achieves the same level of accuracy in practice, so we used backpropagation through a solver in our experiments. 

Here we need to answer two questions:
\begin{itemize}
    \item When is the solution of SDE $\mathrm{d}X_t = f(X_t, t; \theta)\mathrm{d}t + g(X_t, t; \theta)\mathrm{d}W_t$ smooth w.r.t. $\theta$?
    \item When is expectation $\EE_{X_t}[\Lcal(X_t)]$ $L$-smooth w.r.t. $\theta$?
    \begin{itemize}
        \item For example, it is smooth when $\Lcal$ and $X_t$ are both smooth and Lipschitz.
        \item But we often use non-smooth loss function $\Lcal$ (e.g. $x\mapsto \max\{x, 0\}$) in deep hedging for calculating its objective function $\EE[\Lcal(X_T)]$.
        \item Quick Analysis ($x_i=\theta_i, \xi=\{W_t^{(\ell)}\}_{\ell=0}^{\infty}$):
        \begin{align*}
            &\EE_\xi \left\|\nabla \Delta_\ell \hat F(x_1, \xi) - \nabla \Delta_\ell \hat F(x_2, \xi) \right\|^2 
            \\
            &\leq \EE_\xi \left\|
                \nabla \hat F_\ell(x_1, \xi)
                - \nabla \hat F_\ell(x_2, \xi)
                - \nabla \hat F_\infty(x_1, \xi) 
                + \nabla \hat F_\infty(x_2, \xi) 
            \right\|^2 
       \end{align*} 
       This looks hard to bound by $\Ocal(2^{-d\ell}\|x_1 - x_2\|)$.
       \item Assume that the function $\nabla F$ has bounded discontinuity so that $B:=\sup_{x_1, x_2, \xi}\|\nabla \hat F(x_1, \xi) - \nabla \hat F(x_2, \xi) \|$ and $\nabla F(\cdot, \xi)$ is $L$-smooth almost everywhere for any $\xi$. Then, we have
        \begin{align*}
            &\EE_\xi \left\|\nabla \hat F(x_1, \xi) - \nabla \hat F(x_2, \xi) \right\|^2 
            \\
            &\leq L\|x_1 - x_2\| 
            + B \cdot \sup_{\|y_1 - y_2\|\leq \|x_1 - x_2\|} \PP_\xi\left[\text{there exists a discontinuous point of }\nabla \hat F(\cdot, \xi)\text{ on the line between }y_1\text{ and }y_2.\right]
            \\
            &\leq L\|x_1 - x_2\| 
            + B \cdot \sup_{\|y_1 - y_2\|\leq \|x_1 - x_2\|} \PP_\xi\left[\|\nabla \hat F(y_1, \xi) - \nabla \hat F(y_2, \xi)\| > L\right]
        \end{align*}
    \end{itemize}
    \item A milestone would be to prove that 
    \begin{equation*}
    \EE \left\|
        \left(X_T^{\theta_1, \ell} - X_T^{\theta_2, \ell}\right) 
        - \left(X_T^{\theta_1, \infty} - X_T^{\theta_2, \infty}\right) 
    \right\|^2
    \leq 2^{-d\ell}\|\theta_1 - \theta_2\|^2
    \end{equation*}
    \item It might be useful to consider the following coupled SDEs of $X_t:=X^{\theta_1}_t$ and $Y_t:=X^{\theta_2}_t$ 
    \begin{align*}
        \mathrm{d}X_t &= f_X \mathrm{d}W_t + g_X \mathrm{d}t,
        \\
        \mathrm{d}Y_t &= f_Y \mathrm{d}W_t + g_Y \mathrm{d}t.
    \end{align*}
    Considering the SDEs of $X_t+Y_t, X_t-Y_t$ instead, we get
    \begin{align*}
        \mathrm{d}(X_t + Y_t) &= (f_X + f_Y) \mathrm{d}W_t + (g_X + g_Y) \mathrm{d}t,
        \\
        \mathrm{d}(X_t - Y_t) &= (f_X - f_Y) \mathrm{d}W_t + (g_X - g_Y) \mathrm{d}t.
    \end{align*}
    Indeed, the derivative free Milstein scheme of both pairs of SDEs are equivalent because its update rule (with step size $h$) is linear as
    \begin{align*}
        X_{n+1} &= X_n + f_n h + g_n\Delta W_n + \frac{1}{2\sqrt{h}}[g(\bar X_n) - g_n][(\Delta W_n)^2 - h] \\
        \bar X_n &= X_n + f_n h + g_n \sqrt{h} \\
        \Delta W_n &= [W_{(n+1)h} - W_{nh}] \sim N(0, h).
    \end{align*}
\end{itemize}
\end{remark}

